Wide-Depth-Range 6D Object Pose Estimation in Space

6D pose estimation in space poses unique challenges that are not commonly encountered in the terrestrial setting. One of the most striking differences is the lack of atmospheric scattering, allowing objects to be visible from a great distance while complicating illumination conditions. Currently available benchmark datasets do not place a sufficient emphasis on this aspect and mostly depict the target in close proximity. Prior work tackling pose estimation under large scale variations relies on a two-stage approach to first estimate scale, followed by pose estimation on a resized image patch. We instead propose a single-stage hierarchical end-to-end trainable network that is more robust to scale variations. We demonstrate that it outperforms existing approaches not only on images synthesized to resemble images taken in space but also on standard benchmarks.

==> fig/approach.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[t]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.45\linewidth]{./fig/approch/baseline.pdf}&
\includegraphics[width=0.45\linewidth]{./fig/approch/ours.pdf}\\
(a) & (b) \\
\end{tabular}
\caption{{\bf Two different approaches.} (a) Resizing image patches before passing them to a regressor. (b) Our multi-scale approach. \YH{TODO: figure redraw}}
\label{fig:approach}
\end{figure*}

==> fig/motiv.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
    \begin{center}
    % \begin{tabular}{cc}
    % \includegraphics[width=0.45\linewidth, clip, trim=100 10 80 20]{./fig/motivation/1.png} &
    % \includegraphics[width=0.45\linewidth, clip, trim=100 10 80 20]{./fig/motivation/2.png} \\
    % (a) & (b) \\
    % \end{tabular}
    % \fbox{\rule{0pt}{2in} \rule{\linewidth}{0pt}}
    % 
    % https://tex.stackexchange.com/questions/16519/adding-space-between-columns-in-a-table
    \addtolength{\tabcolsep}{-5pt}  % whose value is usually 6pt
    \begin{tabular}{cccc}
    \includegraphics[width=0.24\linewidth]{./fig/motivation/scene_000022_0000.jpg}&
    \includegraphics[width=0.24\linewidth]{./fig/motivation/scene_000002_0005.jpg}&
    \includegraphics[width=0.24\linewidth]{./fig/motivation/scene_000018_0010.jpg}&
    \includegraphics[width=0.24\linewidth]{./fig/motivation/scene_000003_0054.jpg}\\
    % \includegraphics[width=0.24\linewidth,trim=250 200 250 300,clip]{./fig/motivation/scene_000022_0000.jpg}&
    % \includegraphics[width=0.24\linewidth,trim=300 300 300 300,clip]{./fig/motivation/scene_000002_0005.jpg}&
    % \includegraphics[width=0.24\linewidth,trim=500 420 350 430,clip]{./fig/motivation/scene_000018_0010.jpg}&
    % \includegraphics[width=0.24\linewidth,trim=420 450 480 450,clip]{./fig/motivation/scene_000003_0054.jpg}\\
    3d & 8d & 20d & 30d \\
    \end{tabular}
    \addtolength{\tabcolsep}{5pt}  % restore previous value
    % 
    \end{center}
    \vspace{-6mm}
    \caption{{\bf The general 6D object pose estimation VS wide-depth-range.} bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla blabla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla }
    \label{fig:motivation}
\end{figure}

==> fig/real_capture_setting.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.6\linewidth]{./fig/real_capture_setting/input.jpg}
    % \fbox{\rule{0pt}{2in} \rule{0.25\linewidth}{0pt}}
    \end{center}
    \vspace{-6mm}
    \caption{{\bf Demonstration of the Real setting.} bla bla bla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla blabla bla.}
    \label{fig:render_setting}
\end{figure}

==> fig/real_results.tex <==
 % !TEX root = ../top.tex
% !TEX spellcheck = en-US


\begin{figure}[t]
\begin{minipage}{\linewidth}
\centering
\includegraphics[height=2.2cm,trim=450 350 380 50,clip]{fig/swisscube_vs_speed_demo/008982.jpg}
\hspace{1em}
\includegraphics[height=2.2cm,trim=300 450 350 400,clip]{fig/swisscube_vs_speed_demo/scene_000003_0050.jpg}
\begin{scriptsize}
\begin{tabular}{C{0.35\linewidth}C{0.6\linewidth}}
(a) The SPEED dataset & (b) The proposed CubeSat dataset
% (c)&(d)
\end{tabular}
\end{scriptsize}

\vspace{-6mm}
\caption{\small {\bf Comparison of datasets.} {\bf (a)} The SPEED dataset~\cite{Kisantal20} is non-physics-based and only poorly reflecting the complexity of illumination in space {\bf (b)} We propose a physically-based one. The dataset name is temporarily anonymized as CubeSat for not revealing authorship.
}
\label{fig:swisscube_vs_speed_demo}
\end{minipage}
\end{figure}

==> fig/swisscube_demo.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.6\linewidth]{./fig/swisscube_demo/scene_000017_0031.jpg}
    % \fbox{\rule{0pt}{2in} \rule{0.25\linewidth}{0pt}}
    \end{center}
    \vspace{-6mm}
    \caption{{\bf An example from the generated CubeSat dataset.} Note the complex lighting of CubeSat and the twilight zone on the Earth generated by the physical modeling of the whole scene including the Sun, Earth and the CubeSat itself. More can be found in Fig.~\ref{fig:results_demo}.}
    \label{fig:render_setting}
\end{figure}


==> fig/swisscube_earth_renders_L1.tex <==
% !TEX root = ../supp.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
    \centering
    \begin{tabular}{ccc}
    \includegraphics[height=2.4cm]{fig/swisscube_earth_renders_L1/earth_L1_albedo_texture.png}&
    \includegraphics[height=2.4cm]{fig/swisscube_earth_renders_L1/earth_L1_spectral_texture.png}&
    \includegraphics[height=2.4cm]{fig/swisscube_earth_renders_L1/earth_L1_DSCOVR.png}\\
    (a)&(b)&(c)\\
    \end{tabular}
    \vspace{-3mm}
    \caption{\small {\bf Rendered Earth compared to DSCOVR photograph.} (a) Ground-level albedo texture doesn't account for the scattering effects introduced by the atmosphere, resulting in over saturated colors when viewed from space. (b) Rendering of the Earth using our spectral texture based on the VIIRS data products. (c) Ground-truth real photograph taken by the DSCOVR satellite at the L1 Lagrange point.}
    \label{fig:swisscube_earth_renders}
\end{figure}

==> fig/swisscube_stars_envmap.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=1.0\linewidth]{./fig/swisscube_stars_envmap/stars_envmap.jpeg}
    % \fbox{\rule{0pt}{2in} \rule{0.25\linewidth}{0pt}}
    \end{center}
    \vspace{-6mm}
    \caption{{\bf Astronomical objects environment map based on the HYG dataset.} 
    }
    \label{fig:swisscube_stars_envmap}
\end{figure}


==> fig/swisscube_statistics.tex <==
 
 
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.6\linewidth]{./fig/swisscube_statistics/swisscube_statistics.pdf}
    % \fbox{\rule{0pt}{2in} \rule{0.25\linewidth}{0pt}}
    \end{center}
    \vspace{-6mm}
    \caption{{\bf The depth distribution of the target object in datasets.} 
    Nearly 80\% of the SPEED dataset is located in the depth range of 1 to 5 times the object diameter. As contrast, our Swisscube dataset is uniformly distributed among the depth range approximately. Here, the depth is in the unit of times of the diameter of the target object, and note that, we do not have the accurate 3D object model of SPEED, its diameter is approximately computed from a 3D reconstruction. \YH{Suppose to remove this figure, no space}
    }
    \label{fig:swisscube_statistics}
\end{figure}


==> fig/swisscube_sun_spectrum.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=1.0\linewidth]{./fig/swisscube_sun_spectrum/sun_spectrum_plot.jpeg}
    % \fbox{\rule{0pt}{2in} \rule{0.25\linewidth}{0pt}}
    \end{center}
    \vspace{-6mm}
    \caption{{\bf Air mass zero solar spectral power distribution.} 
    }
    \label{fig:swisscube_sun_spectrum}
\end{figure}


==> table/swisscube_stoa.tex <==
 
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
    \centering
    \begin{small}
    % \rowcolors{2}{white}{gray!10}
    \begin{tabular}{lcccc}
        \toprule
        &	Near & Medium & Far & All\\
        \midrule
        {\bf Ours} & {\bf 60.8} & {\bf 51.6} & {\bf 35.1} & {\bf 49.0} \\
        Chen {\it etc.} & 56.7 & 48.2 & 32.8 & 46.1 \\
        SegDriven-Z & 52.6 & 45.4 & 29.4 & 43.2 \\ 
        % \midrule
        \bottomrule
    \end{tabular}
    \end{small}
    \vspace{-3mm}
    \caption{{\bf Comparison with the state of the art on CubeSat.} bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla a bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla v, much more faster as shown in Table~\ref{tab:swisscube_stoa}.}
    \label{tab:swisscube_stoa}
\end{table} 

==> table/swisscube_vs_speed.tex <==
 
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
    \centering
    \begin{small}
    % \rowcolors{2}{white}{gray!10}
    \begin{tabular}{lcc}
        \toprule
        &	SPEED & {\bf CubeSat}\\
        \midrule
        % Synthetic  &12k & 40k \\
        % Real       & 5 & 300 \\
        % \midrule
        Size & 12k & 40k \\
        Accurate 3D model   &\xmark  & \cmark  \\
        Complex lighting    &\xmark  & \cmark \\
        Physical modeling    &\xmark  & \cmark \\
        Colors        &\xmark  & \cmark \\
        Sequences         &\xmark  & \cmark  \\
        Depth distribution & non-uniform & uniform \\
        \bottomrule
    \end{tabular}
    \end{small}
    % \vspace{-3mm}
    \caption{{\bf CubeSat dataset.} bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla bla }
    \label{tab:swisscube_vs_speed}
\end{table} 
